Generating Move Smart Contracts based on Concepts

The growing adoption of formal verification for smart contracts has spurred the development of new verifiable languages like Move. However, the limited availability of training data for these languages hinders effective code generation by large language models (LLMs). This paper presents ConMover, a novel framework that enhances LLM-based code generation for Move by leveraging a knowledge graph of Move concepts and a small set of verified code examples. ConMover integrates concept retrieval, planning, coding, and debugging agents in an iterative process to refine generated code. Evaluations with various open-source LLMs demonstrate substantial accuracy improvements over baseline models. These results underscore ConMover's potential to address low-resource code generation challenges, bridging the gap between natural language descriptions and reliable smart contract development.

==> sections/related.tex <==
\section{Related Work}

\subsection{LLM for Code}

Large language models have shown great promise in automating coding tasks~\cite{wang2021codet5,nijkamp2023codegen2,chaplot2023albert,wei2023magicoder}, from generating code to finding and fixing bugs\cite{jiang2023impact,wu2023effective,xia2023automated,hossain2024deep}. However, current research primarily concentrates on generating correct code in a single attempt. This approach overlooks the importance of iterative refinement, a key aspect of real-world software development where code is continuously revised and improved.

\subsection{Self-Repair}

Previous research has explored using LLMs to improve their own code by either providing them with the results of running the code or training them to find and fix errors on their own\cite{chen2023teaching,huang2023agentcoder,zhong2024ldb,wang2024intervenor,dong2023self}. However, these methods have limitations, such as relying on human input or providing limited improvements. This work presents a new approach that trains LLMs to not only improve their code but also explain the changes made. This method uses a scalable process to automatically collect training data and employs reward functions that evaluate both the quality of the code and the clarity of the explanations.
